A Real-Time Error Prevention System for Gaze-Based Interaction in Virtual Reality Based on Anomaly Detection

Gaze-based interaction enables intuitive, hands-free control in immersive environments, but remains susceptible to unintended inputs. We present a real-time error prevention system (EPS) that uses a temporal convolutional network autoencoder (TCNAE) to detect anomalies in gaze dynamics during selection tasks. In a visual search task in VR, 41 participants used three gaze-based methods - dwell time, gaze and head direction alignment, and nod - with and without EPS. The system reduced erroneous selections by up to 95% for dwell time and gaze and head, and was positively received by most users. Performance varied for nodding and between individuals, suggesting the need for adaptive systems. Objective metrics and subjective evaluations show that anomaly-based error prevention can improve gaze interfaces without disrupting interaction. These findings demonstrate the potential of anomaly-based error prevention for gaze interfaces and suggest applications in VR, AR, and assistive technologies.

==> Content/RelatedWork_old.tex <==
\section{Related work} % Similar to the anomaly detection paper
%NC:could start even more broad if you want, one sentence of how annoying or how someone has to adapt when a system keeps throwing errors, think of those old people trying to use touch screens on airplanes, accidently truning something on when they don't have to this addresses user experience, then we transition to safety, which is equally important (then proceed to your robots).
Interaction with assistive robotic systems is inherently trust-sensitive, and users' perceptions of errors—whether in frequency or severity—can strongly affect their sense of safety and confidence in the system \cite{robottrust,trustdriving}. Prior research has demonstrated that features derived from eye-tracking data can be used to infer user intention \cite{david2021towards, bovo2020detecting} and detect the occurrence of errors during interaction \cite{severitt2023leveraginggaze, bovo2020detecting, lufthansa}. However, most of these approaches focus primarily on identifying user-initiated mistakes, despite the fact that recognition of system-induced errors is equally critical for maintaining trust and preventing hazardous outcomes.% NC: again, we're following to many of the same sources, what's another perspective to these same problems, who else is working on this shit and lets cite those idiots.

Even in systems with low error rates, a single misinterpretation—such as a robotic arm spilling a hot beverage due to an incorrect trajectory—can result in discomfort or danger for the user. 
%NC: yea this is too similar to like 2 of your previous publications, I know you can get creative :) or remove it and take a new direction
These types of incidents, while rare, can elicit strong negative reactions and degrade the perceived reliability of the system. Notably, eye movement behavior has been shown to reflect such incidents in real time, enabling detection opportunities shortly after, or even before, the user confirms their action.
For instance, \citet{peacock2022gazeinputrecognitionerror} successfully distinguished between input recognition errors and deliberate user actions within 50–550 milliseconds post-selection using linear regression models. Similarly, studies in human-robot interaction have shown that gaze patterns change in response to unexpected system behavior, such as increased fixations on unintended or anomalous areas \cite{roboerrorpred}. Despite this progress, identifying the most informative gaze features within these brief temporal windows remains an open challenge. %any other new sources since 2 years? who's been citing peacock lately?

Recent studies have demonstrated the potential of machine learning to improve gaze-based input by contextualizing gaze behavior within the interaction environment. For example, \citet{shevtsova2025gazebasedinteractionml} shows that machine learning techniques were applied to gaze data with free behavior in a visually complex game environment, resulting in a significant reduction in false alarms and an improvement in user satisfaction—all without explicit intention confirmation. Such results underscore the increasing suitability of data-driven methods for improving gaze-based interaction.

Further, sequence modeling approaches such as Temporal Convolutional Networks (TCNs) have been used to classify user errors and predict intent from raw gaze trajectories, achieving performance levels significantly above chance \cite{sendhilnathan2022detectininputrecognitionerrors}. While effective, these classification-based techniques typically rely on labeled data and predefined error categories.

In contrast, our approach reframes selection errors not as predefined classes, but as anomalies within the continuous temporal gaze signal. By treating errors as rare, statistically distinct events, we align our methodology with established techniques in time series anomaly detection, as surveyed by \citet{schmidl2022anomalydetectionsummary}. In our previous work, we demonstrated a theoretical proof-of-concept for applying anomaly detection algorithms to gaze-based interaction data \cite{severitt2025anomalydetection}. In this study, we extend that foundation by implementing and evaluating anomaly detection models on real gaze recordings from a target selection task in a \ac{vr} environment. 

\textcolor{magenta}{NC: what are some solely user experience studies measuring midas touch? would be interesting what they're finding. how will we squash them with our findings.}
